Kernel Interpolation with Sparse Grids

Structured kernel interpolation (SKI) accelerates Gaussian process (GP) inference by interpolating the kernel covariance function using a dense grid of inducing points, whose corresponding kernel matrix is highly structured and thus amenable to fast linear algebra. Unfortunately, SKI scales poorly in the dimension of the input points, since the dense grid size grows exponentially with the dimension. To mitigate this issue, we propose the use of sparse grids within the SKI framework. These grids enable accurate interpolation, but with a number of points growing more slowly with dimension. We contribute a novel nearly linear time matrix-vector multiplication algorithm for the sparse grid kernel matrix. Next, we describe how sparse grids can be combined with an efficient interpolation scheme based on simplices. With these changes, we demonstrate that SKI can be scaled to higher dimensions while maintaining accuracy.

==> content/checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{} 
  \item Did you describe the limitations of your work?
    \answerYes{ See Section~\ref*{sec:discussion}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{ As our method is an improvement on existing methods 
    therefore it doesn't have any direct negative consquences.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
        \item Did you include complete proofs of all theoretical results?
    \answerYes{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{See Section~\ref{app:experiments}.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See Section~\ref{app:hyperparameters_details}.}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{See Figures ~\ref*{fig:mvm_time_memory_comparison} 
    and ~\ref{fig:function_interpolation_gp_inference_results}.}
        \item Did you include the total amount of 
        compute and the type of resources used 
        (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See ~\ref{app:experiments}.}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{} % {We have used GPyTorch \citet{GPyTorchBM} which is licensed under MIT license.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{ See Section~\ref*{sec:introduction}}.
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{We use only publicly available datasets.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{We use only publicly available datasets.}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
  \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
  \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
  \answerNA{}
\end{enumerate}


\end{enumerate}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> content/supplemental_exp.tex <==

\section{Experiments -- Omitted Details and More Results}
\label{app:experiments}

\subsection{Hyperparameters, optimization and data processing details}
\label{app:hyperparameters_details}

We run our experiments on Quadro RTX 8000 with $48$ GB of memory.
For all experiments, we have used RBF kernel with separate length-scale for each dimension. 
For the optimization marginal log-likelihood, we use Adam optimizer with learning rate $0.1$ for $100$ number of epochs. 
The optimization is stopped if no improvement is observed in the log-likelihood for $5$ consecutive epochs.

For GPyTorch,  CG train and test tolerance are set to $1.0$ and $0.01$, which do not worsen perform in practice. 
Both CG pre-conditioning rank and maximum are 100. Our data is split in the ratio of $4:2:3$ to form train, validation and test splits. 
All UCI datasets are standardized using the training data to have zero mean and unit variance.
For sparse-grid, we explore $ \ell \in [2, 3, 4, 5]$ for Table \ref{table:rmse_on_uci_datasets}. 
For dense-grid with simplicial interpolation, we explored grid points per dimension until we run out of memory. 

\subsection{Resources to reproduce results}
\label{app:reproducing_results}

\paragraph*{Code link:} \url{https://anonymous.4open.science/r/skisg-485E/README.md}

%\paragraph*{Link to download datasets:} https://cims.nyu.edu/\~andrewgw/pattern/.%

\subsection{Another interpolation rule to apply sparse grids to large scale dataset}

Recall that it's the relatively higher number of rectilinear grids used in a sparse grid that slows them down on large scale datasets. 
Analogous to the combination rule, we devise a new interpolation rule that only considers rectilinear grids in $\{ \Omega_{\bv{l}} \mid \norm{\bv{l}}_1 = \ell \mid  
\left( \ell \in \bv{l} \,\,\,  \textsc{or} \,\,\, \ell-1 \in \bv{l} \right) \}$, i.e., $d^2/2 + d$ grids.
Similar to combination interpolation technique, all grid interpolation weights are scaled by one by the total number of grids considered.

We focus on two large datasets with relatively higher dimensions, namely, Houseelectric and Airline datasets. 
Houseelectric has $\approx 2.05$ million data points with dimensionality $d=11$. Similarly, Airline dataset has $\approx 5.92$ million data points with dimensionality $d=8$.
For Houseelectric, Sparse-grid performs comparable to Simplex-GP while being $3.95$X faster. 
For the airline dataset, SKIP and SGPR go out-of-memory while Simplex-GP is slower by more than $4$ orders of magnitude.
These results show that sparse grids when used with simplicial interpolation 
can be effective and efficient for large scale dataset.


\begin{table}[]
\caption{Test root-mean-square error (RMSE) and inference time on two large datasets
with dimensions $d \geq 8$ and $n \geq 1M$. See text for more details on datasets.
All numbers are averaged over 3 trials. $\textsc{OOM}$ is out of memory. 
$\star$ number is taken from \citet{SimplicesGP}.}
\centering
\begin{tabular}{|l|c|c|c|c|}
\hline
Methods  & \multicolumn{2}{c|}{Houseelectric} &\multicolumn{2}{c|}{Airline}\\ \hline
   & RMSE & Time (in secs)  & RMSE & Time (in secs)  \\ \hline
SGPR   & $0.067^{\star}$ & -  & OOM  & - \\ \hline
SKIP  & OOM  & - & OOM  & - \\ \hline
Simplex-GP   &  $\bf{0.078}$ & $0.186$   & $0.922$ & $142.891$ \\ \hline        
Dense-grid   & $0.170$ & $0.263$ & $0.892$  & $0.413$ \\ \hline
Sparse-grid  &  $\bf{0.088}$ &  $\bf{0.047}$ & $\bf{0.832}$ & $\bf{0.003}$ \\ \hline
\end{tabular}
\label{table:rmse_on_uci_datasets}
\end{table}

\subsection{Sparse grid interpolation and GP inference for more synthetic functions.}
\label{app:synthetic_interpolation_gp_inference}

\begin{figure}[]
   \begin{subfigure}{0.45 \textwidth}
   \centering \includegraphics[width=\textwidth, height=40mm]{figures/function_interp_error_11.pdf}
   \end{subfigure}
   \hfill
   \begin{subfigure}{0.45 \textwidth}
   \centering \includegraphics[width=\textwidth, height=40mm]{figures/syn_gp_inf_time_f11.pdf} 
   \end{subfigure}
   \begin{subfigure}{0.45 \textwidth}
     \centering \includegraphics[width=\textwidth, height=40mm]{figures/function_interp_error_13.pdf}
     \end{subfigure}
     \hfill
     \begin{subfigure}{0.45 \textwidth}
     \centering \includegraphics[width=\textwidth, height=40mm]{figures/syn_gp_inf_time_f13.pdf} 
     \end{subfigure}
   \caption{Additional results for two more synthetic functions. See section \ref{app:synthetic_interpolation_gp_inference}, for more details.
   % For $d=10$,both methods with cubic interpolation run out of GPU memory, which is $48$ GB for this experiment.
%    our memory budget.
   }
\label{fig:function_interpolation_gp_task_11}
\end{figure}

